Double Patterns: A Usable Solution to Increase the Security of Android Unlock Patterns

Android unlock patterns remain quite common. Our study, as well as others, finds that roughly 25\% of respondents use a pattern when unlocking their phone. Despite known security issues, the design of the pattern interface remains unchanged since first launch. We propose Double Patterns, a natural and easily adoptable advancement on Android unlock patterns that maintains the core design features, but instead of selecting a single pattern, a user selects two, concurrent Android unlock patterns entered one-after-the-other super-imposed on the same 3x3 grid. We evaluated Double Patterns for both security and usability by conducting an online study with $n=634$ participants in three treatments: a control treatment, a first pattern entry blocklist, and a blocklist for both patterns. We find that in all settings, user chosen Double Patterns are more secure than traditional patterns based on standard guessability metrics, more similar to that of 4-/6-digit PINs, and even more difficult to guess for a simulated attacker. Users express positive sentiments in qualitative feedback, particularly those who currently (or previously) used Android unlock patterns, and overall, participants found the Double Pattern interface quite usable, with high recall retention and comparable entry times to traditional patterns. In particular, current Android pattern users, the target population for Double Patterns, reported SUS scores in the 80th percentile and high perceptions of security and usability in responses to open- and closed-questions. Based on these findings, we would recommend adding Double Patterns as an advancement to Android patterns, much like allowing for added PIN length.

==> tables/blacklist.tex <==
\begin{table*}[h]
  \centering
    \begin{tabular}{ r | c | c | c | c }
    \textbf{Treatment} & \textbf{Participants} & \textbf{Blocklisted Participants} & \makecell{\textbf{Non-Blocklisted} \\ \textbf{Participant Changes}} & \textbf{Final is Ideal Choice} \\
    \midrule
    Control & 209 & -- & 26 (12.4\%) & 183 (87.6\%) \\ 
    \midrule
    Blocklist First & 211 & 70 (33.2\%) & 27 (12.8\%) & 114 (54.0\%) \\
    \midrule
    Blocklist Both & 214 & 19 (8.9\%) & 26 (12.1\%) & 169 (79.0\%)\\
    \midrule
    Ideal Choice & 570 & 25 (4.4\%) & 79 (13.9\%) & 466 (81.8\%) \\
    \end{tabular}
\caption{Participant Blocklist Rates and Change Rate of Ideal Choices}
\label{tab:blocklist-rate}
\end{table*}



==> tables/comp_all.tex <==
\begin{table*}[!h]
\caption{ Of note is our users\rq{} evaluation of how Double Pattern compares to existing methods. Above is a comparison of established pattern users in the survey versus non-pattern users, and how their sentiments differed on this evaluation.}
\label{table:comp_all}

    \centering
    \resizebox{\textwidth}{!}{
	\begin{tabular}{|c|c|c|c|}
	\hline
    \multicolumn{4}{|c|}{\textbf{Device Authentication Comparison Among All Participants vs Established Pattern Users}} \\
    \hline
    & Pattern Users & Non-Pattern Users & \makecell{P Value \\ (Significance < .01)} \\
    \hline
    Number of Participants & 162 (25.6\%) & 472 (74.4\%) & -- \\
    \hline
    \makecell{Double Patterns are a secure way \\ to unlock my personal device} & \makecell{ 4.28 \\  Agree}  & \makecell{ 3.97 \\ Agree} & 2.76e-05 \\
    \hline
    \makecell{Double Patterns are more secure than the original Android \\ Patterns for unlocking my personal device} & \makecell{ 4.20 \\ Agree} & \makecell{ 3.92 \\ Agree} & 2.99e-04 \\
    \hline\makecell{Double Patterns are more secure than 4-digit PIN \\ codes for unlock my personal device} & \makecell{ 4.03 \\ Agree} & \makecell{ 3.66 \\ Agree} & 8.60e-06 \\
    \hline
    \makecell{Double Patterns are more secure than 6-digit PIN \\ codes for unlock my personal device} & \makecell{ 3.56 \\ Agree} & \makecell{ 3.23 \\ NAND} & 2.02e-04 \\
    \hline
    \makecell{Double Patterns are more secure than alpha-numeric \\ passwords for unlocking my personal device} & \makecell{ 3.54 \\ Agree} & \makecell{ 3.18 \\ NAND} & 9.33e-05 \\
    \hline
    \end{tabular}}
\end{table*}


==> tables/dev_num.tex <==
\begin{table}[t]
    \centering
    \resizebox{.9\columnwidth}{!}{%
    \begin{tabular}{ r | c c c | c}
    & Control & BL First & BL Double & \textbf{Total} \\
    \toprule
    No Devices & 0 & 1 & 0 & 1 (0.2\%) \\
    1 Device & 122 & 123 & 129 & 374 (59.0\%) \\
    2 Devices & 66 & 73 & 67 & 206 (32.5\%) \\
    3 Devices & 17 & 10 & 15 & 42 (6.6\%) \\
    4 Devices & 4 & 4 & 3 & 11 (1.7\%) \\
    \bottomrule
    \textbf{Total} & {\bf 209} & {\bf 211} & {\bf 214} & \textbf{634} \\ 
    \end{tabular}
    }
  \caption{Amount of Device Utilization in Participants}
  \label{tab:dev} 
\end{table}


==> tables/patt_freq.tex <==
\begin{table*}[!h]    
	\centering
	\resizebox{\textwidth}{!}{
	\begin{tabular}{|c|c|c|c|c|c|}
	    \multicolumn{6}{c} {\textbf{Most Frequent Component Patterns}} \\
	    \hline
        & Control & Blocklist First & Blocklist Both & Ideal Choice & All \\
		\hline
        \makecell{First \\ Component \\ Pattern
        }&
        \makecell{ \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/first-10-0124678.png}} \\
        \footnotesize{freq = 10} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/first-9-0341.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/first-9-0341.png}} \\
        \footnotesize{freq = 9} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/first-8-0125.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/first-8-0143.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/first-8-01258.png}} \\ 
        \footnotesize{freq = 8} \\
        }&
        \makecell{ \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/first-7-6304258.png}} \\
        \footnotesize{freq = 7} \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/first-6-036741.png}} \\
        \footnotesize{freq = 6} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/first-5-01478.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/first-5-6304852.png}} \\ 
        \footnotesize{freq = 5} \\
        }&
        \makecell{ \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/first-9-0143.png}} \\
        \footnotesize{freq = 9} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/first-8-01258.png}} 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/first-8-03678.png}} \\
        \footnotesize{freq = 8} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/first-7-04852.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/first-7-0124678.png}} \\
        \footnotesize{freq = 7} \\
        }&
        \makecell{ \\
        \frame{\includegraphics[width=1cm]{dpatt-images/ideal/all/first-21-03678.png}} \\
        \footnotesize{freq = 21} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/ideal/all/first-18-0124678.png}} \\
        \footnotesize{freq = 18} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/ideal/all/first-17-01258.png}} \\
        \footnotesize{freq = 17} \\
        }&
        \makecell{ \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/all/first-20-0143.png}} \\
        \footnotesize{freq = 20} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/all/first-17-03678.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/all/first-17-0124678.png}} \\
        \footnotesize{freq = 17} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/all/first-16-01258.png}} \\
        \footnotesize{freq = 16} \\
        } \\
		\hline
        \makecell{Second \\ Component \\ Pattern
        }&
        \makecell{ \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-6-1478.png}} \\
        \footnotesize{freq = 6} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-5-0367.png}} 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-5-03678.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-5-7458.png}} \\
        \footnotesize{freq = 5} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-4-01258.png}} 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-4-1258.png}} 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-4-2587.png}} \\ \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-4-5478.png}}  \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-4-21036.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/control/second-4-25876.png}} \\
        \footnotesize{freq = 4} \\
        }&
        \makecell{ \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-01258.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-03678.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-1452.png}} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-147852.png}} 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-210345876.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-25876.png}} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-3674.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-5478.png}} 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-6347.png}} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-64258.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-6784.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-3-8403.png}} \\
        \footnotesize{freq = 3} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-0345.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-0487.png}} \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-1036.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-1258.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-1478.png}} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-2145.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-2478.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-3154.png}} \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-3157.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-4785.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-7412.png}}  \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-21045.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-21476.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-24587.png}} \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-25840.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-41258.png}} 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-63158.png}}  \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-63452.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-0124678.png}}  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blf/second-2-0125876.png}} \\ 
        \footnotesize{freq = 2} \\
        \footnotesize{\emph{Remaining Patterns with}} \\
        \footnotesize{\emph{Single Occurrence Omitted}} \\
        }& 
        \makecell{ \\ 
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/second-6-1478.png}} \\
        \footnotesize{freq = 6} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/second-5-03678.png}} \\
        \footnotesize{freq = 5} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/second-4-01258.png}}
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/blb/second-4-3476.png}} \\
        \footnotesize{freq = 4} \\
        }&
        \makecell{ \\
        \frame{\includegraphics[width=1cm]{dpatt-images/ideal/all/second-15-1478.png}} \\
        \footnotesize{freq = 15} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/ideal/all/second-14-03678.png}} \\
        \footnotesize{freq = 14} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/ideal/all/second-11-01258.png}} \\
        \footnotesize{freq = 11} \\
        }&
        \makecell{ \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/all/second-14-1478.png}} \\
        \footnotesize{freq = 14} \\
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/all/second-13-03678.png}} \\
        \footnotesize{freq = 13} \\  
        \frame{\includegraphics[width=1cm]{dpatt-images/survey/all/second-11-01258.png}} \\
        \footnotesize{freq = 11} \\
        } \\
        \hline
	\end{tabular}}
    \label{tab:freq2}
    \caption{Pattern Frequency by Treatment (cont.)}
\end{table*}


==> tables/start_end.tex <==


\begin{figure*}
\begin{tabular}{c | c}
\multicolumn{2}{c}{\textbf{Overall}}\\
\toprule
{\em Start Point} & {\em End Point}\\
\includegraphics[width=0.33\linewidth]{figures/startend/all-start.pdf} &
\includegraphics[width=0.33\linewidth]{figures/startend/all-end.pdf}\\
\bottomrule

% \multicolumn{2}{c}{\makecell{\\\textbf{Control}}}\\
% \midrule
% {\em Start Point} & {\em End Point}\\
% \includegraphics[width=0.33\linewidth]{figures/startend/control-start.pdf} &
% \includegraphics[width=0.33\linewidth]{figures/startend/control-end.pdf}\\

% \multicolumn{2}{c}{\makecell{\\\textbf{Blocklist Both}}}\\
% \midrule
% {\em Start Point} & {\em End Point}\\
% \includegraphics[width=0.33\linewidth]{figures/startend/both-start.pdf} &
% \includegraphics[width=0.33\linewidth]{figures/startend/both-end.pdf}\\

% \multicolumn{2}{c}{\makecell{\\\textbf{Blocklist First}}}\\
% \midrule
% {\em Start Point} & {\em End Point}\\
% \includegraphics[width=0.33\linewidth]{figures/startend/first-start.pdf} &
% \includegraphics[width=0.33\linewidth]{figures/startend/first-end.pdf}\\

% \multicolumn{2}{c}{\makecell{\\\textbf{Ideal Choice}}}\\
% \midrule
% {\em Start Point} & {\em End Point}\\
% \includegraphics[width=0.33\linewidth]{figures/startend/ideal-start.pdf} &
% \includegraphics[width=0.33\linewidth]{figures/startend/ideal-end.pdf}\\
\end{tabular}
\caption{Frequence of Start/End Choices Across Treatments.}% \reminder{Maybe only show the All? Kind of the same for all of them}}
\end{figure*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/survey.tex <==

\textbf{\small Mobile Device Usage}
\begin{enumerate}\compresslist
\footnotesize \item How many mobile devices do you use regularly?
\item What brands of smartphone do you use for personal use? (Select all that apply)
\item What biometric do you use {\em most often} to unlock your primary personal smartphone?
\item How do you unlock your primary personal smartphone when you reboot the device or if your biometric fails?
\item What unlock method do you use on your primary personal smartphone?
\end{enumerate}

\textbf{\small Post Creation}
\begin{enumerate}\compresslist
\footnotesize \item I feel that the Double Pattern I created provides adequate security for unlocking my personal device. (Likert Scale)
\item It was difficult for me to select a Double Pattern that I would use to unlock my personal device. (Likert Scale)
\item Everyone has a strategy when choosing their authentication, what was your strategy when choosing a Double Pattern?
\end{enumerate}

\textbf{\small Real World Utilization}
\begin{enumerate}\compresslist
\footnotesize \item In a situation where your biometric fails or your mobile device reboots and you are utilizing a Double Pattern to unlock your personal mobile device, would you use the Double Pattern you selected in this survey, or would you select a different one?
\item You have indicated that you (would use|would not use|are unsure if you would use) the Double Pattern you created in this survey on your personal mobile device. Please expand on your choice here.
\end{enumerate}

